Statistical Program Slicing: a Hybrid Slicing Technique for Analyzing Deployed Software

Dynamic program slicing can significantly reduce the code developers need to inspect by narrowing it down to only a subset of relevant program statements. However, despite an extensive body of research showing its usefulness, dynamic slicing is still short from production-level use due to the high cost of runtime instrumentation. As an alternative, we propose statistical program slicing, a novel hybrid dynamic-static slicing technique that explores the trade-off between accuracy and runtime cost. Our approach relies on modern hardware support for control flow monitoring and a novel, cooperative heap memory tracing mechanism combined with static program analysis for data flow tracking. We evaluate statistical slicing for debugging on 21 failures from 6 widely deployed applications and show it recovers 94% of the program statements on a dynamic slice with only 5% overhead.

==> background.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%   SECTION 2   %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Section 2. Challenges of Dynamic Program Slicing
%
% \begin{itemize}
%     \item slice accuracy (solution: slice refinement)
%     \item execution overhead (solution: sampling)
%     \item storage overhead (solution: compress / collapse data dependency edges)
% \end{itemize}
%
\section{Background and Definitions}
\label{sec:background}

In this section, we informally introduce some useful terminology related to program slicing.

\emph{Program slices} include all program statements that might affect a certain instruction of interest, referred to as a \emph{slicing criterion} or \emph{seed}~\cite{manu07}. 
The mechanism for obtaining a slice is by iteratively computing the transitive closure of control and data dependencies between program statements starting from the target instruction.

\emph{Static program slicing} relies on static analysis to conservatively infer potential dependencies between program statements. In contrast, \emph{dynamic program slicing} relies on runtime information gathered during the \emph{particular} execution for which the slice is computed.

Program slices consists of \emph{data and control dependencies} which together define a \emph{program dependency graph} (PDG) \cite{horwitz98}.
Here, nodes correspond to program statements and arcs represents dependence between them.

In the spirit of PDG, we introduce the \emph{observed dependency graph} (ODG) as a program abstraction to aggregate execution information over multiple executions of the same application.
An observed dependency graph consists of control and data dependencies that were exercised (i.e., \emph{observed}) in at least one past monitored program execution. 
Conceptually, the ODG is an unsound approximation of the PDG.


==> tables/table-1.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{lrrrr}
\textbf{App. name} & \textbf{Version} & \textbf{Size (SLoCs)} & \textbf{\# of bugs tested} \\ \hline \hline

%% Gzip %%
gzip & 1.3.12 & 9,081 & 1 \\

%% SQLite %%
sqlite3 & 3.8.0 & 134,283 & 5 \\

%% Curl %%
curl & 7.20.10 & 13,146 & 1 \\

%% Python %%
python & 2.7.11 & 109,311 & 4 \\

%% Cppcheck %%
cppcheck & 1.52 & 358,128 & 5 \\

%% Clang %%
clang & 3.8.0 & 922,201 & 5

\end{tabular}
 \vspace{0.05in} \hrule \vspace{0.025in}
\caption%
{\textbf{Benchmarks summary}. Failures are collected from public bug repositories (e.g., Bugzilla). Application sizes are measured in lines of source code using \texttt{cloc}\protect\footnote{http://cloc.sourceforge.net}.}
\label{table:t1-bugs}
\end{table}

==> tables/table-3.tex <==
\begin{table*}[!t]
\setlength{\tabcolsep}{1em}
\small
\centering
\begin{tabular}{lrrrrr}
Input (\#) & Prec (SLoC) & Wok-SI (SLoC) & Acc-SI (\%) & \
Wok-MI (SLoC) & Acc-MI (\%) \\ \hline \hline

%% Gzip %%
\gzipAname & \aGzipPrecProj & \aGzipWokIdealProj & \
\aGzipAccuracyIdealProj & \aGzipWokStatProj & \aGzipAccuracyStatProj \\ \hline

%% SQLite %%
\sqltAname & \aSqlitePrecProj & \aSqliteWokIdealProj & \
\aSqliteAccuracyIdealProj & \aSqliteWokStatProj & \aSqliteAccuracyStatProj \\

% \bSqliteInput & \bSqlitePrecProj & \bSqliteWokIdealProj & \
% \bSqliteAccuracyIdealProj & \bSqliteWokStatProj & \bSqliteAccuracyStatProj \\

\sqltBname & \cSqlitePrecProj & \cSqliteWokIdealProj & \
\cSqliteAccuracyIdealProj & \cSqliteWokStatProj & \cSqliteAccuracyStatProj \\

\dSqliteInput & \dSqlitePrecProj & \dSqliteWokIdealProj & \
\dSqliteAccuracyIdealProj & \dSqliteWokStatProj & \dSqliteAccuracyStatProj \\

\eSqliteInput & \eSqlitePrecProj & \eSqliteWokIdealProj & \
\eSqliteAccuracyIdealProj & \eSqliteWokStatProj & \eSqliteAccuracyStatProj \\ \hline

%% Curl %%
\aCurlInput & \aCurlPrecProj & \aCurlWokIdealProj & \
\aCurlAccuracyIdealProj & \aCurlWokStatProj & \aCurlAccuracyStatProj \\ \hline

%% Python %%
\aPythonInput & \aPythonPrecProj & \aPythonWokIdealProj & \
\aPythonAccuracyIdealProj & \aPythonWokStatProj & \aPythonAccuracyStatProj \\

\bPythonInput & \bPythonPrecProj & \bPythonWokIdealProj & \
\bPythonAccuracyIdealProj & \bPythonWokStatProj & \bPythonAccuracyStatProj \\

\cPythonInput & \cPythonPrecProj & \cPythonWokIdealProj & \
\cPythonAccuracyIdealProj & \cPythonWokStatProj & \cPythonAccuracyStatProj \\

\dPythonInput & \dPythonPrecProj & \dPythonWokIdealProj & \
\dPythonAccuracyIdealProj & \dPythonWokStatProj & \dPythonAccuracyStatProj \\ \hline

%% Cppcheck %%
\aCppcheckInput & \aCppcheckPrecProj & \aCppcheckWokIdealProj & \
\aCppcheckAccuracyIdealProj & \aCppcheckWokStatProj & \aCppcheckAccuracyStatProj \\ \hline

%% Clang %%
\aClangInput & \aClangPrecProj & \aClangWokIdealProj & \
\aClangAccuracyIdealProj & \aClangWokStatProj & \aClangAccuracyStatProj \\

\bClangInput & \bClangPrecProj & \bClangWokIdealProj & \
\bClangAccuracyIdealProj & \bClangWokStatProj & \bClangAccuracyStatProj \\

\cClangInput & \cClangPrecProj & \cClangWokIdealProj & \
\cClangAccuracyIdealProj & \cClangWokStatProj & \cClangAccuracyStatProj \\

\dClangInput & \dClangPrecProj & \dClangWokIdealProj & \
\dClangAccuracyIdealProj & \dClangWokStatProj & \dClangAccuracyStatProj \\

\eClangInput & \eClangPrecProj & \eClangWokIdealProj & \
\eClangAccuracyIdealProj & \eClangWokStatProj & \eClangAccuracyStatProj \\

\end{tabular}
\vspace{0.125in} \hrule \vspace{0.025in}
\caption{\textbf{Evaluation of statistical program slicing (dynamic slices projected onto source code)}. Slice sizes are measured in source lines of code. As before, numbers are arranged from left to right in decreasing order of precision.}
\label{table:t3-proj-slice}
\end{table*}


==> tables/table-5.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{lrrrrr}

Input (\#) & Prec & WokFR & Ratio & WokCP & Ratio \\
 & (SLoC) & (SLoC) &  & (SLoC) &  \\ \hline \hline

%% Gzip %%
\aGzipInput & \aGzipPrecTail & \aGzipWokIdealTail & \
\aGzipIdealTailRatio & \aGzipWokStatTail & \aGzipStatTailRatio \\ \hline

%% SQLite %%
\aSqliteInput & \aSqlitePrecTail & \aSqliteWokIdealTail &
\aSqliteIdealTailRatio & \aSqliteWokStatTail & \aSqliteStatTailRatio \\

%\bSqliteInput & \bSqlitePrecTail & \bSqliteWokIdealTail &
%\bSqliteIdealTailRatio & \bSqliteWokStatTail & \bSqliteStatTailRatio \\

\cSqliteInput & \cSqlitePrecTail & \cSqliteWokIdealTail &
\cSqliteIdealTailRatio & \cSqliteWokStatTail & \cSqliteStatTailRatio \\

\dSqliteInput & \dSqlitePrecTail & \dSqliteWokIdealTail &
\dSqliteIdealTailRatio & \dSqliteWokStatTail & \dSqliteStatTailRatio \\

\eSqliteInput & \eSqlitePrecTail & \eSqliteWokIdealTail &
\eSqliteIdealTailRatio & \eSqliteWokStatTail & \eSqliteStatTailRatio \\ \hline

%% Curl %%
\aCurlInput & \aCurlPrecTail & \aCurlWokIdealTail & \
\aCurlIdealTailRatio & \aCurlWokStatTail & \aCurlStatTailRatio \\ \hline

%% Python %%
\aPythonInput & \aPythonPrecTail & \aPythonWokIdealTail &
\aPythonIdealTailRatio & \aPythonWokStatTail & \aPythonStatTailRatio \\

\bPythonInput & \bPythonPrecTail & \bPythonWokIdealTail &
\bPythonIdealTailRatio & \bPythonWokStatTail & \bPythonStatTailRatio \\

\cPythonInput & \cPythonPrecTail & \cPythonWokIdealTail &
\cPythonIdealTailRatio & \cPythonWokStatTail & \cPythonStatTailRatio \\

\dPythonInput & \dPythonPrecTail & \dPythonWokIdealTail &
\dPythonIdealTailRatio & \dPythonWokStatTail & \dPythonStatTailRatio \\ \hline

%% Cppcheck %%
\aCppcheckInput & \aCppcheckPrecTail & \aCppcheckWokIdealTail & \
\aCppcheckIdealTailRatio & \aCppcheckWokStatTail & \aCppcheckStatTailRatio \\ \hline

%% Clang %%
\aClangInput & \aClangPrecTail & \aClangWokIdealTail &
\aClangIdealTailRatio & \aClangWokStatTail & \aClangStatTailRatio \\

\bClangInput & \bClangPrecTail & \bClangWokIdealTail &
\bClangIdealTailRatio & \bClangWokStatTail & \bClangStatTailRatio \\

\cClangInput & \cClangPrecTail & \cClangWokIdealTail &
\cClangIdealTailRatio & \cClangWokStatTail & \cClangStatTailRatio \\

\dClangInput & \dClangPrecTail & \dClangWokIdealTail &
\dClangIdealTailRatio & \dClangWokStatTail & \dClangStatTailRatio \\

\eClangInput & \eClangPrecTail & \eClangWokIdealTail &
\eClangIdealTailRatio & \eClangWokStatTail & \eClangStatTailRatio \\

\end{tabular}
\vspace{0.125in}
\hrule
\vspace{0.025in}
\caption{\textbf{Root cause diagnosis quality}. We compare the size of each slice in decrease order of precision (the left--most column showing numbers for precise slice). Except for \texttt{python-2}, all slices include the root--cause.}
\label{table:t5-rootcause}
\end{table}

